Energy Flow in Particle Collisions

In this thesis, I introduce a new bottom-up approach to quantum field theory and collider physics, beginning from the observable energy flow: the energy distribution produced by particle collisions. First, I establish a metric space for collision events by comparing their energy flows. I unify many ideas spanning multiple decades, such as observables and jets, as simple geometric objects in this new space. Second, I develop a basis of observables by systematically expanding in particle energies and angles, encompassing many existing observables and uncovering new analytic structures. I highlight how the traditional criteria for theoretical calculability emerge as consistency conditions, due to the redundancy of describing an event using particles rather than its energy flow. Finally, I propose a definition of particle type, or flavor, which makes use of only observable information. This definition requires refining the notion of flavor from a per-event label to a statistical category, and I showcase its direct experimental applicability at colliders. Throughout, I synthesize concepts from particle physics with ideas from statistics and computer science to expand the theoretical understanding of particle interactions and enhance the experimental capabilities of collider data analysis techniques.

==> appf.tex <==
\chapter{Sample Dependence in Parton Shower Events}
\label{sec:sampledependence}

\begin{figure}[p]
\centering
\includegraphics[scale=.66]{figures/QG_Mass_Hist}
\includegraphics[scale=.66]{figures/QG_Mult_Hist}

\includegraphics[scale=.66]{figures/QG_N95_Hist}
\includegraphics[scale=.66]{figures/QG_Nsd_Hist}

\includegraphics[scale=.66]{figures/QG_Width_Hist}
\includegraphics[scale=.66]{figures/QG_Nsub2_Hist}

\caption{Distributions for the six individual jet observables for $Z$+jet quarks (solid blue), $Z$+jet gluons (solid red), dijet quarks (dashed blue), and dijet gluons (dashed red). 
%
That the quark and gluon histograms for the two different samples are remarkably similar for this array of observables indicates a high degree of sample independence, at least for the notion of quarks and gluons in \pythia.}
\label{fig:qgobshists}
\end{figure}


In this appendix, I do a study of sample dependence of \pythia-labeled quark and gluon jets arising from the $Z+$jet and dijets processes.
%
While this is largely tangential to the main direction of the paper, it lends evidence that our case study is not far from the limit of factorized and universal notions of ``quark'' and ``gluon'' jets.
%
Of course, these conclusions are limited by the fact that they come from jets generated in \pythia, which itself relies on notions of factorization in its generation process.
%
A study of these effects in data would be an important addition to our understanding of sample independence and factorization more broadly.
%
We leave a study using our flavor definition to probe sample dependence in a more realistic collider setting to future work.


In \Fig{fig:qgobshists}, we plot distributions for the six individual substructure observables, from both the $Z$+jet and dijet samples, showing the distributions separately for quarks and gluons as labeled by the \pythia hard scattering process.
%
Importantly, these distributions show a high degree of sample independence: the $Z$+jet and dijet quarks and gluons have very similar distributions.
%
In \Fig{fig:qgmodelhists}, we plot the distributions of the trained model outputs for quarks and gluons from both the dijet and $Z$+jet samples.
%
Similar to the standard jet observables in \Fig{fig:qgobshists}, a high degree of sample independence is observed.
%
This is perhaps more surprising than for the individual observables because these models have the ability to pick up on very slight differences as part of their training.
%
The observed amount of sample independence is encouraging for using CWoLa and jet topics with complicated models.

\begin{figure}[p]
\centering
\includegraphics[scale=.66]{figures/QG_PFP_Hist}
\includegraphics[scale=.66]{figures/QG_PFN_Hist}

\includegraphics[scale=.66]{figures/QG_EFN_Hist}
\includegraphics[scale=.66]{figures/QG_EFP_Hist}

\includegraphics[scale=.66]{figures/QG_CNN_Hist}
\includegraphics[scale=.66]{figures/QG_DNN_Hist}
\caption{Same as \Fig{fig:qgobshists} but for the six trained model outputs.}
\label{fig:qgmodelhists}
\end{figure}
%\afterpage{\clearpage}


For completeness, we also show ROC curves for each of the observables and trained models in \Fig{fig:rocs}, calibrated using the \pythia fractions.
%
Specifically, we use the \pythia-labeled quark fractions of the $Z$+jet and dijet samples to calibrate the classifier ROC curve via \Eqs{eq:epb}{eq:eps}.
%
In \Fig{fig:rocs-obs}, we show ROC curves for each individual observable.
%
In \Fig{fig:rocs-model}, we show ROC curves for each of the trained models.

\clearpage

\begin{figure}[t]
\centering
\subfloat[]{\includegraphics[scale=.755]{figures/ObservableRocs}\label{fig:rocs-obs}}
\subfloat[]{\includegraphics[scale=.755]{figures/ModelRocs}\label{fig:rocs-model}}
\caption{
%
ROC curves for (a) the individual jet observables and (b) the different models trained in the CWoLa paradigm to discriminate $Z$+jet and dijets events. 
%
These are calibrated using \pythia truth fractions.
%
The two best models are PFN-ID and EFPs, which are essentially on top of each other.
}
\label{fig:rocs}
\end{figure}


==> biblio.tex <==
%% This defines the bibliography file (main.bib) and the bibliography style.
%% If you want to create a bibliography file by hand, change the contents of
%% this file to a `thebibliography' environment.  For more information 
%% see section 4.3 of the LaTeX manual.
\begin{singlespace}
\bibliography{main}
\bibliographystyle{plain}
\end{singlespace}


==> signature.tex <==
% -*- Mode:TeX -*-
%
% Some departments (e.g. Chemistry) require an additional cover page
% with signatures of the thesis committee.  Please check with your
% thesis advisor or other appropriate person to determine if such a 
% page is required for your thesis.  
%
% If you choose not to use the "titlepage" environment, a \newpage
% commands, and several \vspace{\fill} commands may be necessary to
% achieve the required spacing.  The \signature command is defined in
% the "mitthesis" class
%
% The following sample appears courtesy of Ben Kaduk <kaduk@mit.edu> and
% was used in his June 2012 doctoral thesis in Chemistry. 

\begin{titlepage}
\begin{large}
This doctoral thesis has been examined by a Committee of the Department
of Chemistry as follows:

\signature{Professor Jianshu Cao}{Chairman, Thesis Committee \\
   Professor of Chemistry}

\signature{Professor Troy Van Voorhis}{Thesis Supervisor \\
   Associate Professor of Chemistry}

\signature{Professor Robert W. Field}{Member, Thesis Committee \\
   Haslam and Dewey Professor of Chemistry}
\end{large}
\end{titlepage}


